MIAShield: Defending Membership Inference Attacks via Preemptive Exclusion of Members

In membership inference attacks (MIAs), an adversary observes the predictions of a model to determine whether a sample is part of the model's training data. Existing MIA defenses conceal the presence of a target sample through strong regularization, knowledge distillation, confidence masking, or differential privacy. We propose MIAShield, a new MIA defense based on preemptive exclusion of member samples instead of masking the presence of a member. The key insight in MIAShield is weakening the strong membership signal that stems from the presence of a target sample by preemptively excluding it at prediction time without compromising model utility. To that end, we design and evaluate a suite of preemptive exclusion oracles leveraging model-confidence, exact or approximate sample signature, and learning-based exclusion of member data points. To be practical, MIAShield splits a training data into disjoint subsets and trains each subset to build an ensemble of models. The disjointedness of subsets ensures that a target sample belongs to only one subset, which isolates the sample to facilitate the preemptive exclusion goal. We evaluate MIAShield on three benchmark image classification datasets. We show that MIAShield effectively mitigates membership inference (near random guess) for a wide range of MIAs, achieves far better privacy-utility trade-off compared with state-of-the-art defenses, and remains resilient against an adaptive adversary.

==> commented-stuff.tex <==
\section{Commented Stuff from Old Version}
\textbf{Chain of Exclusion Oracle vs. Single Exclusion Oracles} For \textbf{Probability-dependent attacks and gap attacks}, the adversary is non-adaptive. As a result, we find the accuracy of exclusion oracles is close. COE shows comparatively less EO accuracy than ESE and ASE ($~.1$) for those settings, which is negligible and does not have much effect on model privacy-utility performance (source: \ref{tab:EO Acc NonM:Prob}). The reason behind this small degradation is, In COE, as all the non-members are by default evaluated by CBE, some non-members are misclassified as members. However, this number of misclassification is very low. Note that, if a non-member is misclassified as a member, intuitively the privacy will not be affected, only this misclassification has some effect on utility (as the number of ensemble models is lower). We can observe this utility loss of COE is $~.2$ compared to ASE/ESE.

\par For label-dependent attacks, we only evaluate the effect of COE vs. the rest of the techniques concerning privacy guarantees only, as we assume the utility is measured in terms of the non-manipulated test dataset. We can observe that attack advantage is dropped up to $~.005$ to $.01$ for COE compared to the rest of the exclusion oracles, especially for boundary distance attacks. Even, attack AUC is dropped $~2\%$ for some cases (source: \ref{tab:EO Acc :Label}). As, if some members are missed by the previous technique, it is captured by the last exclusion oracle system in COE, which increases the privacy guarantee. As the difference of exclusion oracle accuracy of ASE and CBE is comparatively lower over different manipulations, and our defense is not completely dependent on EO accuracy, this privacy improvement is small, but still visible. 

%begin Figures
\begin{comment}
\begin{figure}[t!]
\includegraphics[width=\columnwidth]{figs/Related_Work_AlexNetCifar10_AttackAdv.pdf}
\vspace{-2em}
\caption{Attack Advantage for Logistic Regression(LR) Attack for leading defense techniques with CIFAR-10 dataset and AlexNet Model Architecture }
\label{fig:related_alexnet_cifar10Attack}
\end{figure}

\begin{figure}[t!]
\includegraphics[width=\columnwidth]{figs/Related_Work_AlexNetCifar10_Utility.pdf}
\vspace{-2em}
\caption{Model Utility for Logistic Regression (LR) Attack for leading defense techniques with CIFAR-10 dataset and AlexNet Model Architecture}
\label{fig:related_alexnet_cifar10Utility}
\end{figure}


%%Figure
\begin{figure}[t!]
\includegraphics[width=\columnwidth]{figs/Related_Work_AlexNetCIFAR100_AttackAdv.pdf}
\vspace{-2em}
\caption{Attack Advantage for Logistic Regression(LR) Attack for leading defense techniques with CIFAR-100  dataset and AlexNet Model Architecture }
\label{fig:related_alexnet_CIFAR-100 Attack}
\end{figure}

\begin{figure}[t!]
\includegraphics[width=\columnwidth]{figs/Related_Work_AlexNetCIFAR100_Utility.pdf}
\vspace{-2em}
\caption{Utility loss for Logistic Regression(LR) Attack for leading defense techniques with CIFAR-100  dataset and AlexNet Model Architecture }
\label{fig:related_alexnet_CIFAR-100 util}
\end{figure}

\begin{figure}[t!]
\includegraphics[width=\columnwidth]{figs/Related_Work_AlexNetCH_AttackAdv.pdf}
\vspace{-2em}
\caption{Attack Advantage for Logistic Regression(LR) Attack for leading defense techniques with CH-MNIST dataset and AlexNet Model Architecture }
\label{fig:related_alexnet_CHAttack}
\end{figure}

%%%%%%%EO ACC%%%%%%%%%%
%\begin{comment}
\begin{figure}[t!]
\includegraphics[width=\columnwidth]{figs/Accuracy_of_EO_rotation.pdf}
\vspace{-2em}
\caption{Exclusion Oracle Accuracy with respect to Rotational Manipulation }
\label{fig:EO_acc_rotation}
\end{figure}
%\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t!]
\includegraphics[width=\columnwidth]{figs/Related_Work_AlexNetCH_Utility.pdf}
\vspace{-2em}
\caption{Utility loss for Logistic Regression(LR) Attack for leading defense techniques with CH-MNIST dataset and AlexNet Model Architecture }
\label{fig:related_alexnet_CHutil}
\end{figure}
\end{comment}


\begin{comment}
\par \textbf{DP-SGD} 
From Table .for CIFAR-10 dataset, we can observe that that the utility loss for our model is $~1\%$ while for DP-SGD, utility loss is $~25\%$. On the otherhand, we can observe that our privacy guarantee is compatible with DP-SGD technique, i.e attack advantage $~.02$. For CIFAR-100  datasets, we can observe our technique shows accuracy improvement by $0.88\%$ while DP-SGD shows accuracy loss of $~20\%$. On the contrary, attack advantage is compatible while we consider the probability-dependent LR attack. For CH-MNIST dataset, the utility loss is little bit higher (i.e $~1.5\%$) compared to other datasets as we implied before, CH-MNIST contain comparatively lower number of samples ($1000$-per model), thus it has slightly notable performance reduction. On the contrary, DP-SGD implies $~22\%$ accuracy loss for this dataset as well. Analyzing overall performance with respect to two benchmark and one practical dataset, we can imply that, though DP-SGD is a reliable technique and performing similar as our proposed technique in terms of privacy guarantee, it shows notable accuracy degradation in exchange, while our technique ensures lucrative privacy guarantees in terms of very small utility loss.
% Note that, this comparison is over non-manipulated or original images. We have also noticed another limitation of DP-SGD, while we drastically decrease the additional noise, the model utility does not improve that much. For example, by changing the $\epsilon$ value from $10^3$ to $10^4$, the accuracy of the DP-SGD model only increases $1\%$. So, there is not much room for improving the model utility for the DP-SGD technique. But for our technique, we can always improve and mitigate model utility loss using different techniques, for example, feature engineering, data augmentation.
%\par For AlexNet-Cifar10, we can observe results in Table \ref{tab:related_defense_alex}. 
\par \textbf{PATE} For PATE \cite{PATE17}, we can clearly observe that , PATE produces comparatively large attack advantage compared to DPSGD and our proposed technique over all the datasets , i.e attack advantages are $.05, .06, .14$ for Cifar10, CIFAR-100  and CH-MNIST respectively. Though it provides less accuracy loss compared to DP-SGD (within $~6\%$ to $~16\%$), our system still outperforms this technique both in terms of privacy and utility loss.
\par For label-only attacks, we can observe it also mitigate the attacks in some extends. Problem with PATE is, the privacy-accuracy trade-off is inversely proportional. If we increase the number of teacher models, privacy increases but accuracy degradation occurs. For example, CH-MNIST dataset, when $T_n=5$, the accuracy is $79\%$, while attack AUC for label-dependent data augmentation attack is $.56$  and advantage is $.1$. Though it mitigate attack AUC in some extends, it can not be eradicated with small number of teacher models.On the contrary, our system can completely mitigate the attack AUC with similar number of MIA models, as instead of depending on teacher models decision, it eradicate the vulnerable model in a systematic way.
\par \textbf{Model-Stacking} From the result section we can clearly observe that, Model-stacking demands a high accuracy loss thus does not offer much attack advantage degradation compared to our proposed defense mechanism. In fact, for CIFAR-10 dataset, we found this technique has an attack advantage of $.12$, which is the highest attack advantage, while utility loss is $~8\%$. For CIFAR-100  and CIFAR-10 dataset, this utility loss is within $3\%$, though attack advantage values are still very high.

\par \textbf{MemGuard} For MemGuard, From the result section we can clearly observe that, MemGuard offers $0\%$ label loss with high mitigation in probability dependent attack. On the otherhand, for all the datasets our technique shows less/compatible attack advantage compared to MemGuard.
%For MemGuard \cite{MemGuard19} defense, we have used AlexNet as target model similar as our other settings. We add sample noise to the confidence vector such a way, the original label should not be changed but it can mitigate MIA attack.
\par \textbf{MMD+MixUp} Data Augmentation is a part of MMD-regularization process similar to our design. We can observe that both our attack advantage and utility loss is compatible with this technique.

%Begin Figure: Accuracy of Exclusion Oracles%%%%%
%eo2=[99.99,50,50,50,50]
%eo3=[99.99,81.55,64.24,59.21,50]
\end{comment}

%\section{E}

%%%%%%%%%%%%%%%%%%%%%%%%Table for Hash Result%%%%%%%%
\begin{comment}
\begin{table*}[tbh]
    \centering
    \scalebox{.8}{
    \begin{tabular}{rcccccccc}
    \toprule
         \textbf{Dataset}& \textbf{Attack Type}&\textbf{\# EO Type}  & \textbf{\# Acc of EO} & \textbf{\# Test Acc}&\textbf{\# Train Acc} & \textbf{\# Attack AUC} & \textbf{\# t/($x\in M$)} & \textbf{\# t/($x\not\in M$)} \\ \midrule
          CIFAR-10 & $LR$ & Non-Private & $--$ &$70.02\%$&$94\%$& $.65$  & $--$ & $--$ \\ 
          CIFAR-10 & Threshold & SHA-1 & $99.97\%$&$69.18\%$ &$68.62\%$& $.50$  & $.128s$ & $.161s$ \\ 
            CIFAR-10 & LR & SHA-1 & $99.97\%$ &$69.18\%$&$68.62\%$& $.51$  & $.128s$ & $.161s$ \\ 
            CIFAR-10 & Threshold & pHash & $99.98\%$ &$68.56\%$&$69.06\%$& $.51$  & $.181s$ & $.185s$\\
            CIFAR-10 & Threshold & pHash & $99.98\%$ &$68.56\%$&$69.06\%$& $.54$  & $.181s$ & $.185s$\\
            CIFAR-10 & Threshold & pHash+Rot($5$) & $50\%$ &$68.78\%$&$71.96\%$& $.53$  & $.165s$ & $.166s$\\ 
            CIFAR-10 & LR & pHash+Rot($5$) & $50\%$ &$68.78\%$&$71.96\%$& $.53$  & $.165s$ & $.166s$\\
            CIFAR-10 & Threshold & pHash+Mnp($1p$) & $99.98\%$ &$70.18\%$ & $69.46\%$& $.50$  & $.127s$ & $.161s$\\
            CIFAR-10 & LR & pHash+Mnp($1p$) & $99.98\%$ &$70.18\%$&$69.46\%$& $.52$  & $.127s$ & $.161s$\\
            CIFAR-10 & Threshold & pHash+Mnp(brightness) & $75.34\%$ &$67.18\%$&$72.1\%$& $.53$  & $.153s$ & $.17s$\\
            CIFAR-10 & LR & pHash+Mnp(brightness) & $75.34\%$ &$67.18\%$&$72.1\%$& $.54$  & $.153s$ & $.17s$\\
            CIFAR-10 & Threshold & ML(primary) & $91.19\%$ &$68.22\%$&$67.24\%$& $.51$  & $.164$ & $.165$
            \\CIFAR-10 & Logistic Regression & ML(primary) & $91.19\%$ &$68.22\%$&$67.24\%$& $.52$  & $.164$ & $.165$
            \\CIFAR-10 & Threshold & ML(primary)+Mnp(bright) & $79.2\%$ &$63.62\%$&$69.12\%$& $.53$  & $0.184s$ & $.1836$
            \\CIFAR-10 & LR & ML(primary)+Mnp(bright) & $79.2\%$ &$63.62\%$&$69.12\%$& $.53$  & $0.184s$ & $.1836$
            \\CIFAR-10 & Threshold & ML(primary)+Mnp(1p) & $77.29\%$ &$63.98\%$&$69.8\%$& $.53$  & $.186s$ & $.186s$
            \\CIFAR-10 & LR & ML(primary)+Mnp(1p) & $77.29\%$ &$63.98\%$&$69.8\%$& $.54$  & $.186s$ & $.186s$
            \\\\ \bottomrule
         \\
    \end{tabular}}
    \caption{Result Summary of Exclusion Oracle for Different Settings-Cifar10}
    \label{tab:result-summary}
\end{table*}
\vspace{-.2em}
\end{comment}
%%%%%%%%%%%%%%Analysis Result%%%%%%%%%%%%%%%%%
% \subsection{Analysis Results}
% In this section, we briefly evaluate our experimental findings in terms of several benchmarks as well as practical datasets in terms of our evaluation metrics. 
%\subsection{Evaluation over CIFAR-10Dataset}
%As we discussed above, the adversary query the target model with original datasets, i.e images with zero manipulation.For this settings, the training and testing accuracy of target model is $94\%$ and $70.12\%$ respectively.The AUC value of threshold attack is $.61$ and Logistic Regression or LR attack AUC is $.66$. Now, for SHA-1 hash based exclusion oracle or EO-1 that is discussed in \ref{sec: EO_sha}. The accuracy of the oracle to correctly identifying members vs. non-members is $99.9\%$. From table \ref{tab:result-summary} we can observe that, the training and testing accuracy for this settings, where exclusion oracle is set up as \textbf{EO-1},is $68.62\%$ and $69.18\%$. We can observe that the generalization gap for this setting is negligible. Hence, membership attack accuracy should be negligible and gap attack accuracy should be equal to random guessing.Our obtained results support our claims as both threshold attack AUC and LR attack AUC value is $.50$ and $.51$ respectively.
%\par For $\textbf{EO-2}$ or image hash based exclusion oracle, we have used a series of imagehash algorithms, i.e pHash, wHash, dHash. For \textbf{EO-2} with pHash algorithm, the oracle accuracy is $99.98\%$.Training and Testing accuracy are reported as $69.06$ and $68.56$ respectively for this defense setting. The attack AUC is $.51$ and $.54$ for threshold attack and logistic regression attack respectively.
%\par For $\textbf{EO-3}$, where the exclusion oracle is designed based on machine learning classification and thresholding, as described in \ref{sec: exclusion_oracle_ML}, the accuracy of exclusion oracle for this settings is $91.19\%$. Training and testing accuracy for this mechanism are $67.24\%$ and $68.22\%$. As a result, the attack AUC is $.51$ and $.52$ for threshold and LR attack, which seems to be negligible. The above results suggest that for the CIFAR-10 dataset, with $\textbf{EO-3}$, our defense mechanism successfully mitigates the attack near to random guessing with negligible accuracy loss.
%\par \textbf{Possible Attacks} As we have discussed earlier, for our defense mechanism with \textbf{EO-1} is vulnerable to adaptive attack and time-difference attack. As in this settings, we assume that the adversary initiate non-adaptive attack, does not report any result for prior attack. From the table, we can observe the execution time for member and non-member dataset is $.161s$ and $.128s$ which justifies our claim. The defense mechanism with \textbf{EO-2} is vulnerable to only search based timing attack.The defense mechanism with \textbf{EO-3} is not vulnerable to search based timing attack, so we found nearly equal execution time for member and non-member samples, i.e $.184s$and $.1836s$ respectively.
%############################%%%%%%
%\par \textbf{*Take-Away}From the above result, we can also conclude that, if the exclusion oracles accuracy loss is near or equal $0$, i.e it can successfully produce model index values and excludes the model which contains the members in it's training data, the attack advantage is $~0$.

%For \textbf{AlexNet} Model, we can observe from table \ref{fig:related_alexnet_cifar10Utility} that Non-Private Model shows attack AUC and advantage of $.65$ and $.27$ for Threshold attack and $.67$ and $.27$ for Logistic Regression (LR) attack respectively over CIFAR-10 dataset. The table clearly shows that our technique, \sysname successfully mitigate probability based Membership Inference Attack near to baseline/random guessing, i.e attack AUC and advantage is $.49$ and $.03$ for LR attack over CIFAR-10 dataset. For CIFAR-100  dataset, we can observe from the table \ref{fig:related_alexnet_CIFAR-100 util} that our defense technique mitigates attack AUC from $.63$ to $.51$ and advantage from $.2$ to $.03$. For CH-MNIST, though attack advantage is relatively high with our private settings compared to other datasets, i.e $.09$, the attack AUC is reduced to $.51$ from $.7$ which indicates mitigation of attack success due to the presence of our defense technique.  From table \ref{tab:related_defense_ResNet10_cifar10}, for \textbf{ResNet} model and CIFAR-10 dataset, we can clearly observe that our defense technique mitigate both attack AUC and attack advantage for threshold, LR and MLP attack respectively. For example, for MLP attack, the attack AUC and advantage is reduced from $.60$ to $.52$ and $.33$ to $.05$. Another important observation from the table is, the utility for our technique is increase from non-private to private model, i. e increased from $85.28$ to $87.04$. This result indicates that our defense mechanism need not to trade utility in terms of privacy. We have discussed the details in Section \ref{Effect EO}.


%%%%EO with Manipulation
\begin{comment}
\begin{table*}[t!]
    \centering
    % \small
    \begin{tabular}{rccccc}

        \textbf{EO Type}& \textbf{Dataset}& \textbf{EO Acc (1p)} &\textbf{EO Acc (5p)} & \textbf{EO Acc (10p)}& \textbf{EO Acc (15p)} \\ 
        SHA-1 & CIFAR-10 & $49.94\%$ & $50\%$ & $50\%$ & $49.98\%$ \\
        Img-Hash & CIFAR-10 & $.$ & $.$ & $.$ & $.$ \\
        ML-Classifier  & CIFAR-10 & $.$ & $.$ & $.$ & $.$ \\
        Chain of EO  & CIFAR10& $.$ & $.$ & $.$ & $.$ \\
        
       
           
         \\
    \end{tabular}
    \caption{Exclusion Oracle Evaluation:With Manipulations (Rotations) }
    \label{tab:EO Acc withM}
\end{table*}

%%% Results for Different Exclusion Oracle Accuracy%%%%
%%For manipulation, r=[1,5,10,15]
%begin table-Related Work%%%
%%%%%%%%%%%%%%%%%%%%%%%%Table for Hash Result%%%%%%%%
\begin{comment}
\begin{table*}[t!]
    \centering
    % \small
    \begin{tabular}{rccccc}
    \toprule
        \textbf{Defense}& \textbf{Dataset}& \textbf{Attack Type} & \textbf{\# Test Acc}&\textbf{\# Train Acc} & \textbf{\# Attack AUC}  \\ \midrule
        DP-SGD ($\epsilon=10^4$) & CIFAR-10 & Threshold & $56.74\%$ & $59.72\%$ &$.52$\\
        DP-SGD ($\epsilon=10^4$) & CIFAR-10 & LR & $56.74\%$ & $59.72\%$ &$.53$\\
          DP-SGD ($\epsilon=10^3$) & CIFAR-10 & Threshold & $55.2\%$ & $58.9\%$ &$.52$\\
          DP-SGD ($\epsilon=10^3$) & CIFAR-10 & LR & $55.2\%$ & $58.9\%$ &$.52$\\ 
          DP-SGD($\epsilon=10^2$) & CIFAR-10 & Threshold & $47.2\%$ & $50\%$ &$.5$\\ 
          DP-SGD($\epsilon=10^2$) & CIFAR-10 & LR & $47.2\%$ & $50\%$ &$.49$\\
          PATE($\epsilon=10^-1$) & CIFAR-10 & Threshold & $--\%$ & $--\%$ &$--$

            \\\\ \bottomrule
         \\
    \end{tabular}
    \vspace{-2em}
    \caption{Result Summary of Notable Defense Mechanisms Cifar10}
    \label{tab:related_defensecifar10}
\end{table*}
\end{comment}

\begin{comment}
\begin{table*}[t!]
    \centering
    % \small
    \begin{tabular}{rcccccc}
    
        \textbf{Defense}& \textbf{Dataset}& \textbf{Attack Type} & \textbf{\# Test Acc}&\textbf{\# Train Acc} & \textbf{\# Attack AUC}&\textbf{\# Attack Advantage}  \\ \midrule
        Non-Private & CIFAR-10 & Threshold & $68.12\%$ & $94.12\%$ &$.65$ & $.27$\\
        Non-Private & CIFAR-10 & LR & $68.12\%$ & $94.12\%$ &$.67$ & $.28$\\
        Non-Private & CIFAR-10 & MLP & $68.12\%$ & $94.12\%$ &$.68$ & $.31$\\
        %\sysname & CIFAR-10 & Threshold & $61.72\%$ & $59.26\%$ &$.49$ & $.02$\\
        %\sysname & CIFAR-10 & LR & $64.78\%$ & $65.9\%$ &$.55$ & $.09$\\
        \sysname & CIFAR-10 & Threshold & $67.3\%$ & $66.66\%$ &$.49$ & $.03$\\
        \sysname & CIFAR-10 & LR & $67.3\%$ & $66.66\%$ &$.51$ & $.02$\\
        \sysname & CIFAR-10 & MLP & $67.3\%$ & $66.66\%$ &$.51$ & $.03$\\
        %ImgHash(Case-3) & CIFAR-10 & LR & $65.43\%$ & $69.66\%$ &$.54$ & $.13$\\
        %DP-SGD ($\epsilon=1$) & CIFAR-10 & LR & $10.12\%$ & $11.15\%$ &$.51$ &$.02$\\
        DP-SGD ($\epsilon=10^2$) & CIFAR-10 & LR & $43.6\%$ & $44.34\%$ &$.51$ &$.02$\\
        %DP-SGD ($\epsilon=10^4$) & CIFAR-10 & LR & $46.62\%$ & $49.92\%$ &$.52$ &$.06$\\
        %PATE($\epsilon=1$) & CIFAR-10 & LR & $52.24\%$ & $55.8\%$ &$.52$ & $.06$\\
        %PATE($\epsilon=10^2$) & CIFAR-10 & LR & $52.68\%$ & $55.8\%$ &$.54$ & $.09$\\
        PATE($\epsilon=10^-2$) & CIFAR-10 & LR & $52.1\%$ & $55.8\%$ &$.5$ & $.05$\\
        Model-Stacking & CIFAR-10 & LR & $59.9\%$ & $66.1\%$ &$.57$ & $.12$\\
        MemGuard & CIFAR-10 & LR & $67.74\%$ & $94.04\%$ &$.54$ & $.07$\\
        MMD+MixUp & CIFAR-10 & LR & $68.02\%$ & $75.1\%$ &$.52$ & $.056$\\
        %Non-Private & CIFAR-10 & Gap-Attack & $--\%$ & $--\%$ &$--$ & $--$\\
        %SHA-1(Case-2) & CIFAR-10 & Gap-Attack & $--\%$ & $--\%$ &$--$ & $--$\\

            
         \\
    \end{tabular}
    %\vspace{-2em}

    \caption{Result Summary of Notable Defense Mechanisms: Cifar10-AlexNet}
    \label{tab:related_defense_alexnet_cifar10}
    \vspace{1ex}
    %{\raggedright *Case-1: Without augmentation,ensemble: maximum-vote count \par
    %*Case-2:with data augmentation, provide max confidence score  \par
    %*Case-3:with data augmentation, without EO  \par}
\end{table*}

\begin{table*}[t!]
    \centering
    % \small
    \begin{tabular}{rcccccc}
    %\toprule
        \textbf{Defense}& \textbf{Dataset}& \textbf{Attack Type} & \textbf{\# Test Acc}&\textbf{\# Train Acc} & \textbf{\# Attack AUC}&\textbf{\# Attack Advantage}  \\ %\midrule
        Non-Private & CIFAR-10 & Gap-Attack & $68.12\%$ & $94.12\%$ &$.625$ & $.126$\\
        \sysname & CIFAR-10 & Gap-Attack & $66.2\%$ & $68.26\%$ &$.51$ & $.02$\\
        Non-Private & CIFAR-10 & Label-Only(RA) & $68.12\%$ & $94.12\%$ &$.66$ & $.16$\\
        %Non-Private & CIFAR-10 & Label-Only(RA) & $58.24\%$ & $94.74\%$ &$.75$ & $.25$\\
        \sysname & CIFAR-10 & Label-Only(RA) & $67.3\%$ & $66.6\%$ &$.499$ & $.01$\\
        Non-Private & CIFAR-10 & Label-Only(TA) & $58.24\%$ & $94.74\%$ &$.788$ & $.28$\\
        \sysname & CIFAR-10 & Label-Only(TA) & $65.2\%$ & $65.66\%$ &$.502$ & $.02$\\
        %Non-Private($2.5k$) & CIFAR-10 & Label-Only(BA) & $59.12\%$ & $93.4\%$ &$.818$ & $.--$\\
        Non-Private & CIFAR-10 & Label-Only(BA) & $68.12\%$ & $94.12\%$ &$.646$ & $.19$\\
        \sysname & CIFAR-10 & Label-Only(BA) & $65.43\%$ & $65.66\%$ &$.50$ & $.02$\\
           %\\\\ \bottomrule
         \\
    \end{tabular}
    %\vspace{-1em}
    \caption{Result Summary of \sysname : Cifar10-AlexNet over Label-Dependent Attacks}
    \vspace{1ex}
    {\raggedright *RA: Data Rotation Attack  \par 
    *TA: Data Translation Attack  \par
    *BA: Boundary Distance Attack \par}
    \label{tab:labelonly for CIFAR-10 Dataset}
    %\vspace{1ex}
    %{\raggedright *Case-1: Without augmentation,ensemble: maximum-vote count \par
    %*Case-2:with data augmentation, provide max confidence score  \par}
\end{table*}
\end{comment}

\end{comment}

%%%%%%%%%%%%%%%%%CIFAR-10 more accurate model%%%%%%%%%
\begin{comment}
\begin{table*}[t!]
    \centering
    % \small
    \begin{tabular}{rcccccc}
        \textbf{Defense}& \textbf{Dataset}& \textbf{Attack Type} & \textbf{\# Test Acc}&\textbf{\# Train Acc} & \textbf{\# Attack AUC}&\textbf{\# Attack Advantage}  \\ 
        Non-Private & CIFAR-10 & Threshold & $85.287\%$ & $100\%$ &$.67$ & $.37$\\
        Non-Private & CIFAR-10 & LR & $85.287\%$ & $100\%$ &$.69$ & $.31$\\
        Non-Private & CIFAR-10 & MLP & $85.287\%$ & $100\%$ &$.60$ & $.33$\\
        MemGuard & CIFAR-10 & LR & $85.287\%$ & $100\%$ &$.54$ & $.07$\\
        \sysname & CIFAR-10 & LR & $87.04\%$ & $87.02\%$ &$.49$ & $.03$\\
        \sysname & CIFAR-10 & MLP & $87.04\%$ & $87.02\%$ &$.52$ & $.05$\\
        \sysname & CIFAR-10 & Threshold & $87.04\%$ & $87.02\%$ &$.50$ & $.04$\\
         \\
    \end{tabular}
    \vspace{-2em}
    \caption{Result Summary of Notable Defense Mechanisms: ResNet18(without TL)-Cifar10}
    \label{tab:related_defense_ResNet_cifar10}
    \vspace{1ex}
    {\raggedright *Case-1: Without augmentation,ensemble: maximum-vote count \par
    *Case-2:with data augmentation, provide max confidence score  \par
    *Case-3:with data augmentation, without EO  \par}
\end{table*}


%%%Results for CIFAR-100  Datasets%%%%
\begin{table*}[tbh]
    \centering
    % \small
    \begin{tabular}{rcccccc}
    
        \textbf{Defense}& \textbf{Dataset}& \textbf{Attack Type} & \textbf{\# Test Acc} & \textbf{\# Train Acc} & \textbf{\# Attack AUC}&\textbf{\# Attack Advantage}  \\ 
        Non-Private & CIFAR-100  & LR & $38.46\%$ & $52.88\%$ & $.63$ & $.20$\\
        \sysname & CIFAR-100  & LR & $39.34\%$ & $37.94\%$ & $.51$ & $.03$\\
        DP-SGD & CIFAR-100  & LR & $15.18\%$ & $15.44\%$ & $.49$ & $.03$\\
        PATE & CIFAR-100  & LR & $21.96\%$ & $25.26\%$ & $.53$ & $.06$\\
        Model-Stacking & CIFAR-100  & LR & $31.4\%$ & $50.6\%$ & $.61$ & $.16$\\
        MemGuard & CIFAR-100  & LR & $38.46\%$ & $52.88\%$ & $.52$ & $.04$\\
        MMD+MixUp & CIFAR-100  & LR & $39.54\%$ & $52.88\%$ & $.53$ & $.07$\\
       
    \end{tabular}
    \caption{Result Summary of Notable Defenses Compared to our technique: CIFAR-100 -AlexNet}
    \label{tab:related_defense_alexnet}
\end{table*}

%%%%%
\begin{table*}[!t]
    \centering
    % \small
    \begin{tabular}{rcccccc}
    %\toprule
        \textbf{Defense}& \textbf{Dataset}& \textbf{Attack Type} & \textbf{\# Test Acc}&\textbf{\# Train Acc} & \textbf{\# Attack AUC} & \textbf{\# Attack Advantage}\\ %\midrule
        %Non-Private & CIFAR-100  & LR & $36.68\%$ & $89.72\%$ & $.84$ \\
        Non-Private & CIFAR-100  & Gap-Attack & $36.68\%$ & $89.72\%$ &$76.5\%$ & $.26$\\
        \sysname & CIFAR-100  & Gap-Attack & $33.56\%$ & $33.96\%$ &$49.19\%$ & $.023$\\
        Non-Private & CIFAR-100  & Label-Only(RA) & $36.68\%$ & $89.72\%$ &$79.5\%$ & $.29$ \\
        \sysname & CIFAR-100  & Label-Only(RA) & $33.56\%$ & $33.96\%$ &$49.06\%$ & $.03$\\
        Non-Private & CIFAR-100  & Label-Only(TA) & $36.68\%$ & $89.72\%$ &$79.84\%$ & $.59$\\
         \sysname & CIFAR-100  & Label-Only(TA) & $33.56\%$ & $33.96\%$ &$49.1\%$& $.022$\\
        %Non-Private & CIFAR-100  & Label-Only(BA) & $--\%$ & $\%$ &$\%$& $--$ \\
         \sysname & CIFAR-100  & Label-Only(BA) & $33.56\%$ & $33.96\%$ &$50.1\%$& $.0225$ \\
        
           %\\\\ \bottomrule
         \\
    \end{tabular}
    \caption{Result Summary of \sysname : CIFAR-100 -AlexNet over Label-Dependent Attacks}
    \vspace{1ex}
    {\raggedright *RA: Data Rotation Attack  \par 
    *TA: Data Translation Attack  \par
    *BA: Boundary Distance Attack \par}
    \label{tab:related_defense_alexnet for CIFAR-10 Dataset}
    %\vspace{1ex}
    %{\raggedright *Case-1: Without augmentation,ensemble: maximum-vote count \par
    %*Case-2:with data augmentation, provide max confidence score  \par}
\end{table*}
%%%%%%%%%%%%%%%%%CIFAR-100  VGG-16%%%%%%%%%%%%%
\begin{comment}
\begin{table*}[tbh]
    \centering
    % \small
    \begin{tabular}{rcccccc}
    
        \textbf{Defense}& \textbf{Dataset}& \textbf{Attack Type} & \textbf{\# Test Acc} & \textbf{\# Train Acc} & \textbf{\# Attack AUC}&\textbf{\# Attack Advantage}  \\ 
        Non-Private & CIFAR-100  & LR & $68.1\%$ & $100\%$ & $.79$ & $.49$\\
        Non-Private & CIFAR-100  & MLP & $68.1\%$ & $100\%$ & $.801$ & $.51$\\
        Non-Private & CIFAR-100  & Threshold & $68.1\%$ & $100\%$ & $.80$ & $.55$\\
        \sysname & CIFAR-100  & LR & $\%$ & $\%$ & $.$ & $.$\\
        \sysname & CIFAR-100  & MLP & $\%$ & $\%$ & $.$ & $.$\\
        \sysname & CIFAR-100  & Threshold & $\%$ & $\%$ & $.$ & $.$\\
        DP-SGD & CIFAR-100  & LR & $\%$ & $\%$ & $.$ & $.$\\
        PATE & CIFAR-100  & LR & $\%$ & $\%$ & $.$ & $.$\\
        Model-Stacking & CIFAR-100  & LR & $\%$ & $\%$ & $.$ & $.$\\
        MemGuard & CIFAR-100  & LR & $\%$ & $\%$ & $.$ & $.$\\
        MMD+MixUp & CIFAR-100  & LR & $\%$ & $\%$ & $--$ & $.$\\
       
    \end{tabular}
    \caption{Result Summary of Notable Defenses Compared to our technique: CIFAR-100 -VGG16}
    \label{tab:related_defense_vgg_CIFAR-100 }
\end{table*}
\end{comment}

%%%%%CH-MNIST%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table*}[tbh]
    \centering
    % \small
    \begin{tabular}{rcccccc}
    
        \textbf{Defense}& \textbf{Dataset}& \textbf{Attack Type} & \textbf{\# Test Acc} & \textbf{\# Train Acc} & \textbf{\# Attack AUC}&\textbf{\# Attack Advantage}  \\ 
        Non-Private & CH-MNIST & LR & $81.3\%$ & $99.1\%$ & $.70$ & $.32$\\
        Non-Private & CH-MNIST & MLP & $81.3\%$ & $99.1\%$ & $.66$ & $.26$\\
        \sysname & CH-MNIST & LR & $79.8\%$ & $80.05\%$ & $.51$ & $.07$\\
        \sysname & CH-MNIST & MLP & $79.8\%$ & $80.5\%$ & $.51$ & $.07$\\
        DP-SGD($\epsilon=10$ & CH-MNIST & LR & $56.5\%$ & $58\%$ & $.51$ & $.07$\\
        PATE & CH-MNIST & LR & $75.7\%$ & $81.5\%$ & $.56$ & $.14$\\
        Model-Stacking & CH-MNIST & LR & $78.9\%$ & $96.1\%$ & $.60$ & $.18$\\
        MemGuard & CH-MNIST & LR & $81.3\%$ & $99.1\%$ & $.58$ & $.08$\\
        MMD+MixUp & CH-MNIST & LR & $80.4\%$ & $82.07\%$ & $.52$ & $.08$\\
       
    \end{tabular}
    \caption{Result Summary of Notable Defenses Compared to our proposed technique for CHMNIST-AlexNet}
    \label{tab:related_defense_alexnet}
\end{table*}

\begin{table*}[!t]
    \centering
    % \small
    \begin{tabular}{rcccccc}
    %\toprule
        \textbf{Defense}& \textbf{Dataset}& \textbf{Attack Type} & \textbf{\# Test Acc}&\textbf{\# Train Acc} & \textbf{\# Attack AUC} & \textbf{\# Attack Advantage}\\ %\midrule
        Non-Private & CH-MNIST & Gap-Attack & $81.3\%$ & $99.01\%$ &$57.15\%$ & $.145$ \\
        \sysname & CH-MNIST & Gap-Attack & $79.8\%$ & $80.5\%$ &$49.2\%$ & $.015$ \\
        Non-Private & CH-MNIST & Label-Only(RA) & $81.3\%$ & $99.01\%$ &$92.85\%$ & $.857$\\
        \sysname & CH-MNIST & Label-Only(RA) & $79.8\%$ & $80.5\%$ &$52.68\%$ & $.053$ \\
        Non-Private & CH-MNIST & Label-Only(TA) & $81.3\%$ & $99.01\%$ &$89.3\%$ & $.78$\\
        \sysname & CH-MNIST & Label-Only(TA) & $79.8\%$ & $80.5\%$ &$51.3\%$ & $.024$\\
        Non-Private & CH-MNIST & Label-Only(BA) & $81.3\%$ & $99.01\%$ &$64.5\%$ & $.256$ \\
        \sysname & CH-MNIST & Label-Only(BA) & $79.8\%$ & $99.01\%$ &$50.7\%$& $.022$ \\
        
           %\\\\ \bottomrule
         \\
    \end{tabular}
    \caption{Result Summary of \sysname : CH-MNIST-AlexNet over Label-Dependent Attacks }
    \vspace{1ex}
    {\raggedright *RA: Data Rotation Attack  \par 
    *TA: Data Translation Attack  \par
    *BA: Boundary Distance Attack \par}
    \label{tab:related_defense_alexnet for CH-MNIST Dataset}
    %\vspace{1ex}
    %{\raggedright *Case-1: Without augmentation,ensemble: maximum-vote count \par
    %*Case-2:with data augmentation, provide max confidence score  \par}
\end{table*}
\end{comment}

 %On generalization gap vs. AUC plot we can find a strong relationship between generalization gap vs. attack auc as the distance of y axis from baseline increases with the increasing number of generalization gap. Note that, we observe our technique reduces the generalization gap for all the datasets, and this improvement reflects with the improvement of AUC in MIAShield from undefended models. 
%We have evaluated the label-dependent attacks, i.e both label-only and Gap attack for CIFAR-10 dataset in table \ref{tab:labelonly for CIFAR-10 Dataset}. For Cifar10, our proposed technique reduces Gap attack AUC from $.625$ to $.51$. As from the table we can observe that the generalization gap (GP) for \sysname is $.46\%$ while for non-private setting the value of GP is $26\%$. As gap attack success is dependent on GP value, our technique can successfully mitigate this attack by reducing GP in a large amount. We can also observe from the table that the label dependent manipulation based attacks are mitigated by our proposed defense by analyzing both the reduction of attack AUC and attack advantage. For example, attack AUC is reduced from $.75$ to $.499$ for Rotation attack, from $.788$ to $.502$ for data translation attack, and from $.646$ to $.50$ for boundary distance attack. Our exclusion oracle is designed to detect the members even if they are slightly manipulated. Hence, the manipulated images created by the Label-only attacker are detected and excluded by our oracle, thus the attack fails, which is clearly reflected by our results. We can observe similar outcomes for CIFAR-100  and CH-MNIST datasets. For Gap attack, the attack AUC is reduced from $.76$ to $.49$ for CIFAR-100  dataset and from $.57$ to $.49$ for CH-MNIST dataset. On the Contrary, for CIFAR-100  dataset, we can observe our defense technique reduces label-only (RA, TA, BA) attack AUC from $~.8$ to baselinec AUC, i.e $~.5$. For CH-MNIST, attack AUC and attack advantage value is slightly higher in augmentation attack (RA) despite of the presence of our defense mechanism , i.e AUC is $.52$ and advantage is $.053$. (why??).Label-dependent manipulated attacks (label-only attacks) include manipulated images while querying the target model. Our exclusion oracles can detect manipulated images in some extend, which is evaluated in the performance evaluation of EO section. Though they miss the manipulated images in some extend, from result section we can observe that the label-only attack accuracy is still low.The reason behind that is, the attack dataset contains the original image while query the target model, and all our EO system in \sysname (from EO2-EO5) can detect this non-manipulated images. Hence, \sysname provide the result for non-manipulated image, it excludes the model that contains membership signal, thus the attack remains unsuccessful.

%From Table \ref{tab:Related Work:Prob} for CIFAR-10,  dataset, we can observe that that the utility loss DP-SGD is. On the otherhand, , i.e attack advantage $~.02$. For CIFAR-100  datasets, we can observe our technique shows accuracy improvement by $0.88\%$ while DP-SGD shows accuracy loss of $~20\%$. On the contrary, attack advantage is compatible while we consider the probability-dependent LR attack. For CH-MNIST dataset, the utility loss is little bit higher (i.e $~1.5\%$) compared to other datasets as we implied before, CH-MNIST contain comparatively lower number of samples ($1000$-per model), thus it has slightly notable performance reduction. On the contrary, DP-SGD implies $~22\%$ accuracy loss for this dataset as well.
 



\end{comment}


==> context.tex <==
\section{Problem Statement and Threat Model}\label{sec: prob-stmt}
Suppose, there is a big dataset which contains millions of users sensitive data. We will build an MLaaS system that will work as a prediction API in a black-box settings. So for a given input, the
model will produce an prediction output or labels. According to MIA, this type of system is at a risk for data leakage as model can memorize the data/ Overfitting may occur. The intuition behind in this type of attack is, the models act differently when they see the data which was used to train the model. So how we can use this intuition as a defense technique? Obviously differential privacy is a solution. But differential private training can make a system slow and may cause significant accuracy reduction. Now imagine, we split the dataset into $m$ distinct datasets and train $m$ number of models using these data. Our adversary put input $x$ and try to find out whether this data is a member of the training data $D$. So we have $m$ number of models and $x$ is member of one of those models, suppose $m1$. So all the $m$ models will produce prediction vector for input $x$. Then we will try to find these differences of prediction $P_1$ to $P_m$. (I think how to compute this difference will be the challenge). Our intuition is, $P1$ will act differently to input $x$, and the rest $P_2$ to $P_m$ will not act differently. So our output will be the aggregated prediction vector of $P_2$ to $P_m$ and we will avoid the output from $P_1$
\par Note:One reason of membership inference attack is that every classifier contains small number of examples, can we do something about it?
\par Challenges: The major challenge in our work is to identify the vulnerable model with respect to input data $x$. We can think about this as a classification problem like membership inference attack. We have some advantages compared to MIA attack. First, in MIA attack, the attacker only has black box access to the model. As now we are the owner of the model, we can assume that we have white box access to the model and we can use this advantages to identify member/non-members with respect to a model. We can add extra challenges considering that the adversary has white box access to the model. 

